Dr. Strategy: Model-Based Generalist Agents with Strategic Dreaming

Model-based reinforcement learning (MBRL) has been a primary approach to ameliorating the sample efficiency issue as well as to make a generalist agent. However, there has not been much effort toward enhancing the strategy of dreaming itself. Therefore, it is a question whether and how an agent can "dream better" in a more structured and strategic way. In this paper, inspired by the observation from cognitive science suggesting that humans use a spatial divide-and-conquer strategy in planning, we propose a new MBRL agent, called Dr. Strategy, which is equipped with a novel Dreaming Strategy. The proposed agent realizes a version of divide-and-conquer-like strategy in dreaming. This is achieved by learning a set of latent landmarks and then utilizing these to learn a landmark-conditioned highway policy. With the highway policy, the agent can first learn in the dream to move to a landmark, and from there it tackles the exploration and achievement task in a more focused way. In experiments, we show that the proposed model outperforms prior pixel-based MBRL methods in various visually complex and partially observable navigation tasks.

==> algorithms/unsupervised_algo.tex <==
\begin{algorithm}[!ht]
   \caption{\red{Unsupervised Training} \red{WIP}}
   \red{Hany: This is just an approximation of the algorithm high-level, maybe I will go deeper in details or change a bit}
        
    {\bfseries Initialize:} Replay buffer $\mathcal{D}$, World Model $\mathcal{M}$, VQ-VAE \red{(Encoder $\mathbf{E}$, Codebook $\mathbf{C}$, Decoder $\mathbf{D}$)}, \red{Anchors $\mathcal{Z}$}, latent anchor-conditioned policy $\pi_{a}(a_t\vert s_t,z)$, goal-conditioned achiever policy $\pi_{g}(a_t\vert s_t,e_g)$, exploration policy $\pi_{e}(a_t\vert  s_t)$, and other neural networks.

    
    {\bfseries Input:} Curious anchor sampling frequency $\mathcal{F}_a$, Latent anchor-conditioned policy's maximum number of deployment steps $T_\text{anchor}$

    \DontPrintSemicolon

        \While{exploring}{
        % \FOR{$i=1$ {\bfseries to} $T$}
        %     \IF{$i\%T_{\text{sample a curious anchor}}$}
        %         \STATE Imagine trajectories $\tau_{1\hdots \vert \mathcal{Z}\vert}$ using $\mathcal{M}\ \&\ \pi_{e}$ starting from the anchors $\mathcal{Z}$
        %         % \STATE Compute values of the imagined trajectories $V(\tau_j) = \frac{\sum_{t=1}^{T_{\text{imagination}}}\mathbb{E}_{\pi_e}[\sum r_t^e]}{T_{\text{imagination}}}$ (Eq. \ref{section:eq})

        %         \STATE Compute values of the imagined trajectories $V(\tau_{1\hdots \vert \mathcal{Z}\vert}) = \frac{\sum_{t=1}^{T_{\text{imagination}}}\mathbb{E}_{\pi_e}[\sum r_t^e]}{T_{\text{imagination}}}$ (Eq. \ref{section:eq})
        %         % \STATE $z^* \sim  \text{Categorical}(\hat{\mathcal{Z}})$
        %         \STATE $z^* \sim  \text{Categorical}(V(\tau_{1\hdots \vert \mathcal{Z}\vert}))$
        %         % \STATE Compute a Categorical distribution $\hat{\mathcal{Z}}$ based on $V(\tau_{1\hdots \vert \mathcal{Z}\vert})$
        %         % \STATE Compute values of the imagined trajectory Eq. \ref{section:eq} and associating them to the anchors
        %     \ENDIF
        % \ENDFOR
        Sample a mini-batch of trajectories $\mathcal{B} \sim \mathcal{D}$\;
        
        Train $\mathcal{M}$ and VQ-VAE on $\mathcal{B}$\;
        
        Train in imagination $\pi_{a}(a_t|s_t,z)$ (Section \ref{section:}), $\pi_{g}(a_t|s_t,e_g)$ (Section \ref{section:}) and $\pi_{e}(a_t|s_t)$ (Section \ref{section:}) on $\mathcal{B}$\;
        
        \If{should sample a new curious anchor based on frequency $\mathcal{F}_a$?}{
            Imagine trajectories $\tau_{1\hdots \vert \mathcal{Z}\vert}$ using $\mathcal{M}$ with $\pi_{e}$ starting from anchors $\mathcal{Z}$\;
            
            Compute values of the imagined trajectories $V(\tau_{1\hdots \vert \mathcal{Z}\vert})$ (Eq. \ref{section:eq})\;
            %= \frac{\sum_{t=1}^{T_{\text{imagination}}}\mathbb{E}_{\pi_e}[\sum r_t^e]}{T_{\text{imagination}}}$
            
            $z^* \sim  \text{Categorical}(V(\tau_{1\hdots \vert \mathcal{Z}\vert}))$\;
            
            Deploy $\pi_{a}(a_t\vert s_t,z^*)$ in the environment for $T_\text{anchor}$ steps or till $\lVert s_t - s_{z*} \rVert < \epsilon$ and grow $\mathcal{D}$
        }
        Deploy $\pi_{e}(a_t\vert s_t)$ in the environment to explore and grow $\mathcal{D}$ 
        % \IF{should deploy achiever during exploring?}
        %     \STATE \red{From LEXA, paraphrase or remove}
        %     \STATE Get a sampled goal image embedding $e_g$ using $\mathcal{M}$ such that $g \sim \mathcal{D}$ 
        %     \STATE Deploy $\pi_g(a_t\vert s_t, e_g)$ in the environment and grow $\mathcal{D}$.
        % \ENDIF
}   
\end{algorithm}


==> algorithms/zeroshot_algo.tex <==

% \begin{algorithm}[H]
%    \caption{\red{Zero-Shot Adaptation}}
   
%    \label{alg:example}
%     \begin{algorithmic}
        
%         \STATE {\bfseries Input (Trained):} World Model $\mathcal{M}$, VQ-VAE \red{(Encoder $\mathbf{E}$, Codebook $\mathbf{C}$, Decoder $\mathbf{D}$)}, \red{Anchors $\mathcal{Z}$}, anchor-conditioned policy $\pi_{a}(a_t \vert s_t,z)$, goal-conditioned achiever policy $\pi_{g}(a_t\vert s_t,e_g)$

%         \STATE {\bfseries Input:} Goal image $x_g$
%         \STATE {\bfseries Input:} Latent anchor-conditioned policy's maximum number of deployment steps $T_\text{anchor}$


%         \STATE Get the goal image embedding $e_g$ from $x_g$ using $\mathcal{M}$
%         \STATE Get the goal image state $s_g$ from $e_g$ using $\mathcal{M}$
%         \STATE Get the nearest anchor $z^*$ from $s_g$ using VQ-VAE (Section \ref{section:})
%         \STATE Deploy $\pi_{a}(a_t|s_t,z^*)$ in the environment for $T_\text{anchor}$ steps or till $\lVert s_t - s_{z*} \rVert < \epsilon$
%         \STATE Deploy $\pi_g(a_t\vert s_t, e_g)$ in the environment for the remaining steps in the episode
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[!ht]
    \caption{\red{Zero-Shot Adaptation} \red{WIP}}
    {\bfseries Input (Trained):} World Model $\mathcal{M}$, VQ-VAE \red{(Encoder $\mathbf{E}$, Codebook $\mathbf{C}$, Decoder $\mathbf{D}$)}, \red{Landmarks $\mathcal{Z}$}, Landmark-conditioned policy $\pi_{l}(a_t \vert s_t,z)$, Goal-conditioned achiever policy $\pi_{g}(a_t\vert s_t,e_g)$
    
    {\bfseries Input:} Goal image $x_g$
    
    {\bfseries Input:} Latent landmark-conditioned policy's maximum number of deployment steps $T_\text{anchor}$, Episode length $T$\;

    \DontPrintSemicolon

  %     \tcp{this is a comment}
  % \tcc{Now this is an if...else conditional loop}
  % \If{Condition 1}
  %   {
  %       Do something    \tcp*{this is another comment}
  %       \If{sub-Condition}
  %       {Do a lot}
  %   }
    
    Get the goal image embedding $e_g$ from $x_g$ using $\mathcal{M}$\;
    
    Get the goal image state $s_g$ from $e_g$ using $\mathcal{M}$\;
    
    Get the nearest anchor $z^*$ from $s_g$ using VQ-VAE (Section \ref{section:})\;

    $x_t = x_0 \leftarrow \mathrm{Env.reset}()$\;
    
    $s_t = s_0 = 0$\;
 
    $a_t = a_0 = 0$\;
    
    \For{t=0\hdots T-1}
    {
        \text{Get model state using World Model posterior} $s_t \sim q(s_t \vert s_{t-1}, a_{t-1}, x_t)$
        
        \If{$t < T_\text{anchor}\ \text{and}\ \lVert s_t - s_{z*} \rVert > \epsilon$}
        {
            \text{Compute latent landmark-achieving action} $a_t \leftarrow \pi_{l}(a_t|s_t,z^*)$ %\tcp{Latent landmark-conditioned policy}
        }
        \Else{
            \text{Compute goal-achieving action}  $a_t \leftarrow \pi_g(a_t\vert s_t, e_g)$ %\tcp{Goal-conditioned policy}
        }

        $x_t = \mathrm{Env.step}(a_t)$
        % \If{t \geq T_\text{anchor}\ \text{or}\ $\lVert s_t - s_{z*} \rVert < \epsilon$}
        % {
        %     $a_t \leftarrow \pi_g(a_t\vert s_t, e_g)$
        % }
        % \Else{
        %     $a_t \leftarrow \pi_{a}(a_t|s_t,z^*)$
        % }
    }
    
   % \While{episode is not terminated}
   % {
   %      $\pi = $
   % 		Do something\;
   % }
    
    % Deploy $\pi_{a}(a_t|s_t,z^*)$ in the environment for $T_\text{anchor}$ steps or till $\lVert s_t - s_{z*} \rVert < \epsilon$\;
    
    % Deploy $\pi_g(a_t\vert s_t, e_g)$ in the environment for the remaining steps in the episode\;

\end{algorithm}
